The GAN is dead; long live the GAN! A Modern GAN Baseline

There is a widely-spread claim that GANs are difficult to train, and GAN architectures in the literature are littered with empirical tricks. We provide evidence against this claim and build a modern GAN baseline in a more principled manner. First, we derive a well-behaved regularized relativistic GAN loss that addresses issues of mode dropping and non-convergence that were previously tackled via a bag of ad-hoc tricks. We analyze our loss mathematically and prove that it admits local convergence guarantees, unlike most existing relativistic losses. Second, our new loss allows us to discard all ad-hoc tricks and replace outdated backbones used in common GANs with modern architectures. Using StyleGAN2 as an example, we present a roadmap of simplification and modernization that results in a new minimalist baseline -- R3GAN. Despite being simple, our approach surpasses StyleGAN2 on FFHQ, ImageNet, CIFAR, and Stacked MNIST datasets, and compares favorably against state-of-the-art GANs and diffusion models.

==> figures/qualitative/stacked-mnist-3x3.tex <==
{
% Variable to control the size of each image
\begin{figure}[h!]
    \newlength{\imgsize}
    \setlength{\imgsize}{0.2\linewidth} % Adjust this value to change the size of the images
    
    \setlength{\tabcolsep}{0pt} % Remove spacing between columns
    \renewcommand{\arraystretch}{0} % Remove spacing between rows

    % New command to include images from a specific directory
    \newcommand{\qualitativeimg}[1]{%
        \includegraphics[width=\imgsize]{figures/qualitative/stacked-mnist-000008806/number-#1.jpg}%
    }
    \centering
    \includegraphics[width=\imgsize, trim=0px 0px 2048px 2048px]{figures/qualitative/stacked-mnist-000008806.png}
    \caption{qualitative example of stacked-mnist}
    \label{fig:stacked-mnist}
\end{figure}
}

==> figures/tables/imgnet32x32-fid-table.tex <==
\begin{table}[h]
\centering
\caption{FID on ImageNet-32}
\begin{tabular}{ l c c }
\toprule
Model & \textbf{Year} & FID$\downarrow$ \\
\midrule
% %Real NVP (Dinh et al.) & 2016 & 4.28 \\
% %Glow (Kingma and Dhariwal) & 2018 & 4.09 \\
% %MintNet & 2019 & 4.06 \\
% % Residual Flow & 2019 & 4.01 \\
% % BIVA Maaloe et al. & 2019 & 3.96 \\
% % ANF Huang et al. & 2020 & 3.92 \\
% % NVAE w/ flow & 2020 & 3.92 \\
% % PixelRNN & 2016 & 3.86 \\
% % Flow++ & 2019 & 3.86 \\
% % SPN Menick and Kalchbrenner & 2018 & 3.85 \\
% % Gated PixelCNN & 2016 & 3.83 \\
% % Very Deep VAE & 2020 & 3.8 \\
% % MRCNF & 2021 & 3.77 \\
% % $\delta$-VAE & 2019 & 3.77 \\
% Image Transformer~\cite{parmar2018image} & 2018 & 3.77 \\
% ScoreFlow & 2021 & 3.76 \\
% Reflected Diffusion & 2023 & 3.74 \\
% %Hourglass & 2021 & 3.74 \\
% DenseFlow-74-10 & 2021 & 3.63 \\
% i-DODE & 2023 & 3.43 \\
% MSGAN~\cite{karnewar2020msg} & 2019 & 12.3 \\
% DDPM-IP & 2023 & 2.66 \\
MSGAN~\cite{karnewar2020msg} & 2019 & 12.3 \\
VDM~\cite{kingma2021variational} & 2021 & 7.41 \\
DDPM++~\cite{kim2021soft} & 2021 & 8.42 \\
DDPM-IP~\cite{ning2023input} & 2023 & 2.87 \\
\textbf{Ours} & 2024 & 1.28 \\
StyleGAN-XL~\cite{sauer2022stylegan} & 2022 & \textbf{1.10} \\
\bottomrule
\end{tabular}
\end{table}

==> packages-icml.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
\usepackage{booktabs}       % professional-quality tables
\usepackage{array}
% \setlength{\heavyrulewidth}{1.5pt}
% \setlength{\abovetopsep}{4pt}
\usepackage{multirow}

%\usepackage[table]{xcolor}
%\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{siunitx}
\usepackage{xspace}

\usepackage{todonotes}
\usepackage{comment}
\usepackage{amsmath} 

% Type
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage[super]{nth}
\usepackage{floatrow}

% Lists
\usepackage[inline,shortlabels]{enumitem}
%\usepackage{lipsum}
\usepackage{wrapfig}
\usepackage{tikz}
\usetikzlibrary{calc,spy}
% \usepackage[subtle]{savetrees}
\DeclareMathOperator\supp{supp}
\usepackage{cancel}
\usepackage{tabularray}
\usepackage{rotating}
\usepackage{pdflscape}
\usepackage{caption}
\usepackage{wrapfig}

\usepackage{adjustbox}


% \setcitestyle{square}
% \setcitestyle{citesep={,}}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcommand{\upperRomannumeral}[1]{\uppercase\expandafter{\romannumeral#1}}
\newcommand{\lowerromannumeral}[1]{\romannumeral#1\relax}


==> tex/experiments-icml.tex <==
\section{Experiments}
\label{sec:exp}
We evaluate our model on FFHQ ($256\times256$)~\cite{sg1} for high resolution unimodal image synthesis, and high diversity generation on CIFAR-10~\cite{krizhevsky2009learning}, and ImageNet ($32\times32$)~\cite{chrabaszcz2017downsampled}. We compare our model with various baselines, in Table \ref{tab:ffhq256}, \ref{tab:cifar10}, and \ref{tab:imagenet32}.

We leave a detailed discussion of our results in Appendix E. Our model surpasses StyleGAN2 and StyleGAN3 by a large margin across datasets despite its simplicity. Unless with ImageNet feature leakage~\cite{sauer2021projected,kynkaanniemi2022role} or certain regularization~\cite{zhao2021improved} that has been shown to overfit~\cite{zhang2022styleswin} on FFHQ $256\times256$, no GAN comes close to R3GAN in terms of FID. Our model also beats diffusion models despite having a considerably smaller model size and that it generates samples in one step.\looseness=-1 








\vspace{-2ex}

\begin{table}[]
        \begin{tblr}{
          column{2} = {r},
          cell{1}{2} = {c},
          hline{2,5,9,10} = {-}{},
        }
        Model       & FID$\downarrow$  \\
        StyleGAN2   & 3.78 \\
        StyleGAN3-T & 4.81 \\
        StyleGAN3-R & 3.92 \\
        LDM & 4.98\\
        ADM (DDIM) & 8.41\\
        ADM (DPM-Solver) & 8.40\\
        Diffusion Autoencoder & 5.81\\
        Ours---Config E  & 2.77 \\
        \emph{With ImageNet feature leakage~\cite{kynkaanniemi2022role}:} & \\
        PolyINR*~\cite{singh2023polynomial} & 2.72 \\
        StyleGAN-XL*~\cite{sgxl} & 2.19 \\
        StyleSAN-XL*~\cite{takida2024san} & 1.36 \\
        \end{tblr}
        \caption{
        \label{tab:ffhq256}FFHQ-256. * denotes models that leak ImageNet features.}
        \vspace{-0.7cm}
\end{table}

\begin{table}[]
        \vspace{-0.2cm}
        \begin{tblr}{
          column{2} = {r},
          cell{1}{2}{3} = {},
          hline{2,9,13} = {-}{},
        }
        Model               & FID$\downarrow$ \\
        BigGAN~\cite{biggan}              & 14.73 \\
        TransGAN~\cite{trans}            & 9.26 \\
        ViTGAN~\cite{vitgan}              & 6.66 \\
        DDGAN~\cite{ddgan}               & 3.75 \\
        Diffusion StyleGAN2 & 3.19 \\
        StyleGAN2 + ADA     & 2.42 \\
        StyleGAN3-R + ADA   & 10.83 \\
        DDPM               & 3.21 \\
        DDIM                & 4.67 \\
        VE~\cite{edm}                  & 3.11 \\
        VP~\cite{edm}                  & 2.48 \\
        Ours---Config E     & 1.97 \\
        \hline
        \emph{With ImageNet feature leakage~\cite{kynkaanniemi2022role}:} & \\
        StyleGAN-XL*~\cite{sgxl}       & 	1.85 \\
        \end{tblr}
        \caption{\label{tab:cifar10}CIFAR-10.}
        %\vspace{-0.7cm}
\end{table}
\begin{table}[h!]
        \begin{tblr}{
          column{2} = {r},
          cell{1}{2} = {c},
          hline{2,5,9,10} = {-}{},
        }
        Model               & FID$\downarrow$       \\
        \emph{Unconditional} & \\
        DDPM++~\cite{kim2021soft}           & 8.42  \\ % (is unconditional)
        VDM~\cite{kingma2021variational}    & 7.41  \\ % (is unconditional)
        \emph{Conditional} & \\
        MSGAN~\cite{karnewar2020msg}        & 12.3  \\
        ADM~\cite{adm,ning2023input}                      & 3.60  \\
        DDPM-IP~\cite{ning2023input}        & 2.87  \\
        Ours---Config E                     & 1.27  \\ 
        \emph{With ImageNet feature leakage~\cite{kynkaanniemi2022role}:} & \\
        StyleGAN-XL*~\cite{sgxl}            & 1.10  \\
        \end{tblr}
        \caption{\label{tab:imagenet32}ImageNet-32.}
        %\vspace{-0.7cm}
\end{table}

==> tex/loss-icml.tex <==


%------------------------------------------------------------------------
\section{Serving Two Masters: Stability and Diversity with RpGAN \texorpdfstring{$+ R_1+R_2$}{R-1R-2}}
%---An Improved Training Objective \vk{title can be tweaked; i recommend naming your new loss}}
% James Tompkin: I wrote 'serving two masters'. Note that 'serving two masters' is inherently a religious label; in the bible, Matthew writes that one cannot serve two masters (only God). In the traditions of monarchy (to which our title alludes in the procession of kings), a king had divine right and so avoided this problem of serving two masters (to serve God and to serve one's king is to serve two masters, except once we establish that kings are divine then this problem goes away as the same master - God - is then being served). I am not religious.
\label{sec:loss}

In defining a GAN objective, we tackle two challenges: stability and diversity. Some previous work deals with stability~\cite{sg1,sg2,sg3} and other previous work deals with mode collapse \cite{rgan}. We combine a stable method with a simple regularizer grounded by theory to overcome both.

\vspace{-1ex}
\subsection{Traditional GAN}
\vspace{-1ex}
A traditional GAN~\cite{gan,nowozin2016f} is formulated as a minimax game between a discriminator $D_\psi$ and a generator $G_\theta$. Given real data $x\sim p_\mathcal{D}$ and fake data $x\sim p_\theta$ produced by $G_\theta$, the most general form of a GAN is given by:
\begin{align}
\begin{split}
\label{eq:gan}
\resizebox{0.438\textwidth}{!}{$
\mathcal{L}(\theta,\psi)=\mathbb{E}_{z\sim p_z}\left[f\left(  D_\psi(G_\theta(z))\right)\right]+\mathbb{E}_{x\sim p_\mathcal{D}}\left[f\left( -D_\psi(x) \right)\right]
$}
\end{split}
\end{align}
\noindent where $G$ tries to minimize $\mathcal{L}$ while $D$ tries to maximize it. The choice of $f$ is flexible~\cite{lsgan,hingegan}. In particular, $f(t) = -\log(1+e^{-t})$ recovers the classic GAN by Goodfellow~\etal~\cite{gan}. For the rest of this work, this will be our choice of $f$~\cite{nowozin2016f}.

% It is shown that Eq.\ref{eq:gan} is actually convex if we can directly optimize $p_\theta$~\cite{gan,rpgan}. Though in practice, the empirical GAN loss moves fake samples past the decision boundary induced by $D$ rather than updating the density function $p_\theta$ directly. This turns out to be a much harder problem that is susceptible to two common failure cases: mode collapse/dropping\footnote{Mode collapse and mode dropping are technically two related yet distinct problems. We use these two terms interchangeably hereafter to refer to the general problem where $\supp p_\theta$ fails to fully cover $\supp p_\mathcal{D}$.} and non-convergence. \vk{Minor thing: could provide a bit more information (1 sentence) on mode dropping and collapse}
It has been shown that Equation~\ref{eq:gan} has convex properties when $p_\theta$ can be optimized directly~\cite{gan,rpgan}. However, in practical implementations, the empirical GAN loss typically shifts fake samples beyond the decision boundary set by $D$, as opposed to directly updating the density function $p_\theta$. This deviation leads to a significantly more challenging problem, characterized by susceptibility to two prevalent failure scenarios: mode collapse/dropping\footnote{While mode collapse and mode dropping are technically distinct issues, they are used interchangeably in this context to describe the common problem where $\supp\ p_\theta$ does not fully cover $\supp\ p_\mathcal{D}$.} and non-convergence.

\vspace{-1ex}
\subsection{Relativistic \texorpdfstring{$f$-GAN}{f-GAN}.}
\vspace{-1ex}
% We adopt relativistic pairing GAN (RpGAN) by Jolicoeur-Martineau~\etal~\cite{rgan} as the main GAN loss. 
% Sun~\etal showed that RpGAN is especially effective against mode dropping~\cite{rpgan} as the loss landscape of RpGAN contains no local minima that correspond to mode dropping solutions. 
% Next, we apply zero-centered gradient penalties~\cite{r1,r1r2} to RpGAN. Gradient penalty is a well known technique that stabilizes GAN training~\cite{wgan-gp,r1r2,r1} and has been proven to be crucial to GAN convergence~\cite{r1}. As our contribution to the theory, we follow Mescheder~\etal~\cite{r1} and prove that gradient-penalized RpGAN enjoys the same guarantee of local convergence as regularized classic GANs. In addition to theoretical guarantees, our empirical results suggest that gradient penalized RpGAN is sufficiently well-behaved, to the extent that allows us to remove all GAN tricks without encountering non-convergence or mode dropping.

We employ a slightly different minimax game named relativistic pairing GAN (RpGAN) by Jolicoeur-Martineau~\etal~\cite{rgan} to address mode dropping. The general RpGAN is defined as:
\begin{equation}
\label{eq:rpgan}
\mathcal{L}(\theta,\psi)=\mathbb{E}_{\substack{z\sim p_z\\x\sim p_\mathcal{D}}}\left[f\left(  D_\psi(G_\theta(z))-D_\psi(x) \right)\right]
\end{equation}
Although Eq.\ref{eq:rpgan} differs only slightly from Eq.\ref{eq:gan}, evaluating the critic difference has a fundamental impact on the landscape of $\mathcal{L}$. Since Eq.\ref{eq:gan} merely requires $D$ to separate real and fake data, in the scenario where all real and fake data can be separated by a single decision boundary, the empirical GAN loss encourages $G$ to simply move all fake samples barely past this single boundary---this degenerate solution is what we observe as mode collapse/dropping. Sun~\etal~\cite{rpgan} characterize such degenerate solutions as bad local minima in the landscape of $\mathcal{L}$, and show that Eq.\ref{eq:gan} has \emph{exponentially many} bad local minima. The culprit is the existence of a single decision boundary that naturally arises when real and fake data are considered in isolation. RpGAN introduces a simple solution by coupling real and fake data,~\ie a fake sample is critiqued by its realness \emph{relative to} a real sample, which effectively maintains a decision boundary in the neighborhood of \emph{each} real sample and hence forbids mode dropping. Sun~\etal~\cite{rpgan} show that the landscape of Eq.\ref{eq:rpgan} contains no local minima that correspond to mode dropping solutions, and that every basin is a global minimum.

\vspace{-1ex}
\subsection{Training Dynamics of RpGAN}
\vspace{-1ex}
Although the landscape result~\cite{rpgan} of RpGAN allows us to address mode dropping, the training dynamics of RpGAN have yet to be studied. The ultimate goal of Eq.~\ref{eq:rpgan} is to find the equilibrium $(\theta^*,\psi^*)$ such that $p_{\theta^*}=p_\mathcal{D}$ and $D_{\psi^*}$ is constant everywhere on $p_\mathcal{D}$. Sun~\etal~\cite{rpgan} show that $\theta^*$ is globally reachable along a non-increasing trajectory in the landscape of Eq.\ref{eq:rpgan} under reasonable assumptions. However, the existence of such a trajectory does not necessarily mean that gradient descent will find it. Jolicoeur-Martineau~\etal show empirically that unregularized RpGAN does not perform well~\cite{rgan}. 

\vspace{0.5ex}
\noindent \textbf{Proposition~\upperRomannumeral{1}.} (Informal) \emph{Unregularized RpGAN does not always converge using gradient descent.}
%\vk{Propositions should ideally be made precise or in the worst case, say it's an informal statement (but then you still have to make it intuitively understandable)}
\vspace{0.5ex}

\noindent We confirm this proposition with a proof in Appendix H. 
% In summary, we follow Mescheder~\etal~\cite{r1} and inherit their DiracGAN counterexample to apply it to RpGAN. 
We show analytically that RpGAN does not converge for certain types of $p_\mathcal{D}$, such as ones that approach a delta distribution. Thus, further regularization is necessary to fill in the missing piece of a well-behaved loss.

\vspace{-1.5ex}
\paragraph{Zero-centered gradient penalties.}
To tackle RpGAN non-convergence, we explore gradient penalties as the solution since it is proven that zero-centered gradient penalties (0-GP) facilitate convergent training for classic GANs~\cite{r1}. The two most commonly-used 0-GPs are $R_1$ and $R_2$:
\begin{equation}
\begin{aligned}
R_1(\psi)&=\frac{\gamma}{2}\mathbb{E}_{x\sim p_\mathcal{D}}\left[\left\| \nabla_x D_\psi \right \|^2\right]\\ 
R_2(\theta,\psi)&=\frac{\gamma}{2}\mathbb{E}_{x\sim p_\theta}\left[\left\| \nabla_x D_\psi \right \|^2\right]
\end{aligned}
\end{equation}
$R_1$ penalizes the gradient norm of $D$ on real data, and $R_2$ on fake data. Analysis on the training dynamics of GANs has thus far focused on local convergence~\cite{nagarajan2017gradient,gannum,r1},~\ie whether the training at least converges when $(\theta,\psi)$ are in a neighborhood of $(\theta^*,\psi^*)$. In such a scenario, the convergence behavior can be analyzed~\cite{nagarajan2017gradient,gannum,r1} by examining the spectrum of the Jacobian of the gradient vector field $\left(-\nabla_\theta\mathcal{L},\nabla_\psi\mathcal{L} \right )$ at $(\theta^*,\psi^*)$. The key insight here is that when $G$ already produces the true distribution, we want $\nabla_x D=0$, so that $G$ is not pushed away from its optimal state, and thus the training does not oscillate. $R_1$ and $R_2$ impose such a constraint when $p_\theta=p_\mathcal{D}$. This also explains why earlier attempts at gradient penalties, such as the one-centered gradient penalty (1-GP) in WGAN-GP~\cite{wgan-gp}, fail to achieve convergent training~\cite{r1} as they still encourage $D$ to have a non-zero slope when $G$ has reached optimality.

Since the same insight also applies to RpGAN, 
we extend our previous analysis and show that:
% our goal is to extend the proof of Mescheder~\etal~\cite{r1} to RpGAN and show that:

\vspace{0.5ex}
\noindent \textbf{Proposition~\upperRomannumeral{2}.} (Informal) \emph{RpGAN with $R_1$ or $R_2$ regularization is locally convergent subject to similar assumptions as in} Mescheder~\etal~\cite{r1}.
\vspace{0.5ex}

In Appendix I, our proof similarly analyzes the eigenvalues of the Jacobian of the regularized RpGAN gradient vector field at $(\theta^*,\psi^*)$. We show that all eigenvalues have a negative real part; thus, regularized RpGAN is convergent in a neighborhood of $(\theta^*,\psi^*)$ for small enough learning rates~\cite{r1}.

\vspace{-1ex}
\paragraph{Discussion.}
Another line of work~\cite{r1r2} links $R_1$ and $R_2$ to instance noise~\cite{instancenoise} as its analytical approximation. Roth et al.~\cite{r1r2} showed that for the classic GAN~\cite{gan} by Goodfellow~\etal, $R_1$ approximates convolving $p_\mathcal{D}$ with the density function of $\mathcal{N}(0, \gamma I)$, up to additional weighting and a Laplacian error term. $R_2$ likewise approximates convolving $p_\theta$ with $\mathcal{N}(0, \gamma I)$ up to similar error terms. The Laplacian error terms from $R_1$, $R_2$ cancel when $D_\psi$ approaches $D_{\psi^*}$. We do not extend Roth~\etal's proof~\cite{r1r2} to RpGAN; however, this approach might provide complimentary insights to our work, which follows the strategy of Mescheder~\etal~\cite{r1}. 

We demonstrate our loss in Appendix A where we focus on practical considerations such as global convergence. Building on Roth et al.~\cite{r1r2}, we apply both $R_1$ and $R_2$ to improve global stability.

==> tex/roadmap-icml.tex <==
% \begin{figure}
%     \centering
%     \includegraphics{figures/FID-vs-Params-Plot.eps}
%     \caption{This scatter-plot shows the FID performance of our model on FFHQ-256 vs the number of parameters when only trained for 5million steps}
%     \label{fig:fid-vs-params-ablation}
% \end{figure}


\section{A Roadmap to a New Baseline --- \modelName}
\label{sec:roadmap}

% \vk{What about naming the new GAN that is being proposed? SimpleGAN...?}\jt{R3GAN...?}

% \vk{My main comment about this section is that it reads like mix of methods and experiments: all the experimental details/results (e.g., we set the learning rate to $10^{-4}$) should be under experiments (but you can still describe the key important takeaways here, e.g., we need a smaller learning rate)}

The well-behaved RpGAN + $R_1$ + $R_2$ loss alleviates GAN optimization problems, and lets us proceed to build a minimalist baseline---\modelName---with recent network backbone advances in mind~\cite{convnext,metaformer}. Rather than simply state the new approach, we will draw out a roadmap from the StyleGAN2 baseline~\cite{sg2ada}. This model (Config A; identical to~\cite{sg2ada}) consists of a VGG-like~\cite{vgg} backbone for $G$, a ResNet $D$, a few techniques that facilitate style-based generation, and many tricks that serve as patches to the weak backbone. Then, we remove all non-essential features of StyleGAN2 (Config B), apply our loss function (Config C), and gradually modernize the network backbone (Config D-E).


We evaluate each configuration on FFHQ $256\times256$~\cite{sg1}. Network capacity is kept roughly the same for all configurations---both $G$ and $D$ have about 25M trainable parameters. Each configuration is trained until $D$ sees 5M real images. We inherit training hyperparameters (optimizer settings, batch size, EMA decay length,~\etc) from Config A unless otherwise specified. We tune the training hyperparameters for our final model and show the converged result in Sec.~\ref{sec:exp}.

%\paragraph{StyleGAN2 (Config A).}This configuration is identical to the baseline~\cite{sg2ada} with the style-based generator and all tricks enabled.  

\vspace{-1ex}
\paragraph{Minimum Baseline (Config B).}
We strip away all StyleGAN2 features, retaining only the raw network backbone and basic image generation capability. The features fall into three categories:
\begin{itemize}[leftmargin=10pt,itemsep=0pt,topsep=0pt]
\item Style-based generation: mapping network~\cite{sg1}, style injection~\cite{sg1}, weight modulation/demodulation~\cite{sg2}, noise injection~\cite{sg1}.
\end{itemize}\quad % JT: Weird but intential LaTeX
\begin{itemize}[leftmargin=10pt,itemsep=0pt,topsep=0pt]
\vspace{-0.25cm} % JT: Weird but intential LaTeX
\item Image manipulation enhancements: mixing regularization~\cite{sg1}, path length regularization~\cite{sg2}.
\item Tricks: $z$ normalization~\cite{pggan}, minibatch stddev~\cite{pggan}, equalized learning rate~\cite{pggan}, lazy regularization~\cite{sg2}.
\end{itemize}

% Such features could be reintroduced as per application need (e.g., style injection). 
Following~\cite{sgxl,sg-t}, we reduce the dimension of $z$ to 64. The absence of equalized learning rate necessitates a lower learning rate, reduced from $2.5\times10^{-3}$ to $5\times10^{-5}$. Despite a higher FID of 12.46 than Config-A, this simplified baseline produces reasonable sample quality and stable training. We compare this with DCGAN~\cite{dcgan}, an early attempt at image generation. Key differences include:
\begin{enumerate}[label=\alph*), noitemsep,topsep=0pt,leftmargin=24pt]
\item Convergent training objective with $R_1$ regularization.\label{item:convergent} 
\item Smaller learning rate, avoiding momentum optimizer (Adam $\beta_1=0$).\label{item:learning_rate} 
\item No normalization layer in $G$ or $D$.\label{item:normalization} 
\item Proper resampling via bilinear interpolation instead of strided (transposed) convolution.\label{item:resampling} 
\item Leaky ReLU in both $G$ and $D$, no tanh in the output layer of $G$.\label{item:activation} 
\item $4\times4$ constant input for $G$, output skips for $G$, ResNet $D$.\label{item:input} 
\end{enumerate}

We discuss our findings about these principles in Appendix B and establish that \ref{item:convergent} through \ref{item:activation} are critical to the success of StyleGAN2, and apply them to all subsequent configurations.

\paragraph{Well-behaved loss function (Config C).}
% Given the simplified baseline, we move on to the modernization part of the roadmap. We first modernize the loss function so that the representation power of modern network backbones will not be compromised by GAN optimization difficulties. 
We use the loss function proposed in Section~\ref{sec:loss} and this reduces FID to 11.65. We hypothesize that the network backbone in Config B is the limiting factor. 
% and expect more drastic improvements as further modernization takes place.

\paragraph{General network modernization (Config D).}
First, we apply the 1-3-1 bottleneck ResNet architecture~\cite{resnet,resnet2} to both $G$ and $D$. This is the direct ancestor of all modern vision backbones~\cite{convnext,metaformer}. 
% However, rather than precisely replicating the architecture in~\cite{resnet2}, 
We also incorporate principles discovered in Config B and various modernization efforts from ConvNeXt~\cite{convnext}. We categorize the roadmap of ConvNeXt as follows:
% \begin{enumerate}[label=\roman*)]
%     \item Consistently beneficial: 1) increased width with depthwise conv. 2) inverted bottleneck. 3) fewer activation functions. 4) separate resampling layers.
%     \item Negligible performance gain: 1) large kernel depthwise conv with fewer channels. 2) replacing ReLU with GELU. 3) fewer normalization layers. 4) replacing batch norm with layer norm.
%     \item Irrelevant to our problem setting: 1) improved training recipe. 2) stage ratio. 3) "patchify" stem.
% \end{enumerate}
% % We are interested in applying i) to our model, among which i.3) and i.4) are applicable to the classic ResNet. We leave i.1) and i.2) for Config E. Much of ii) were introduced merely for the sake of mimicking vision transformers~\cite{swin,vit} even though they fail to bring any significant improvement~\cite{convnext}. ii.3) and ii.4) are inapplicable since we do not use any normalization layer following principle c). ii.2) is directly at odds with our finding that GELU deteriorates GAN performance, and we use leaky ReLU as in principle e). Liu~\etal put heavy emphasis on using large conv kernels (ii.1)~\cite{convnext}, however this results in slightly but consistently worse performance than using wider $3\times3$ conv layers and we therefore do not employ this design choice of ConvNeXt.

% We aim to apply i) to our model, specifically i.3) and i.4) for the classic ResNet, while reserving i.1) and i.2) for Config E. Many aspects of ii) were introduced merely to mimic vision transformers~\cite{swin,vit} without yielding significant improvements~\cite{convnext}. ii.3) and ii.4) are inapplicable due to our avoidance of normalization layers following principle c). ii.2) contradicts our finding that GELU deteriorates GAN performance, thus we use leaky ReLU per principle e). Liu~\etal emphasize large conv kernels (ii.1)~\cite{convnext}, but this results in slightly worse performance compared to wider $3\times3$ conv layers, so we do not adopt this ConvNeXt design choice.
%
\begin{enumerate}[label=\roman*., itemsep=2pt,leftmargin=12pt,topsep=0pt]
    \item Consistently beneficial: \begin{enumerate*}[label=\theenumi\arabic*), ref=\arabic*, before=\unskip{ }, itemjoin={{, }}, itemjoin*={{, and }}]
        \item\label{item:i1} increased width with depthwise conv.
        \item\label{item:i2} inverted bottleneck
        \item\label{item:i3} fewer activation functions
        \item\label{item:i4} separate resampling layers
    \end{enumerate*}
    \item Negligible performance gain: \begin{enumerate*}[label=\theenumi\arabic*), ref=\arabic*, before=\unskip{ }, itemjoin={{, }}, itemjoin*={{, and }}]
        \item\label{item:ii1} large kernel depthwise conv.~with fewer channels
        \item\label{item:ii2} swap ReLU with GELU
        \item\label{item:ii3} fewer normalization layers
        \item\label{item:ii4} swap batch norm.~with layer norm.
    \end{enumerate*}
    \item Irrelevant to our setting: \begin{enumerate*}[label=\theenumi\arabic*), ref=\arabic*, before=\unskip{ }, itemjoin={{, }}, itemjoin*={{, and }}]
        \item\label{item:iii1} improved training recipe
        \item\label{item:iii2} stage ratio
        \item\label{item:iii3} ``patchify'' stem
    \end{enumerate*}
\end{enumerate}

We aim to apply i) to our model, specifically i.\ref{item:i3} and i.\ref{item:i4} for the classic ResNet, while reserving i.\ref{item:i1} and i.\ref{item:i2} for Config E. Many aspects of ii) were introduced merely to mimic vision transformers~\cite{swin,vit} without yielding significant improvements~\cite{convnext}. ii.\ref{item:ii3} and ii.\ref{item:ii4} are inapplicable due to our avoidance of normalization layers following principle c). ii.\ref{item:ii2} contradicts our finding that GELU deteriorates GAN performance, thus we use leaky ReLU per principle e). Liu~\etal emphasize large conv kernels (ii.\ref{item:ii1})~\cite{convnext}, but this results in slightly worse performance compared to wider $3\times3$ conv layers, so we do not adopt this ConvNeXt design choice. We discuss the architecture details in Appendix C.

\begin{figure}[t]
    \includegraphics[width=\linewidth,clip,trim={87pc 0cm 0cm 0cm}]{figures/network.pdf}
    \caption{Network architecture blocks.}
    \label{fig:network}
    \vspace{-0.7cm}
\end{figure}

\paragraph{Bottleneck modernization (Config E).}
Now that we have settled on the overall architecture, we investigate how the residual block can be modernized, specifically i.\ref{item:i1}) and i.\ref{item:i2}). First, we explore i.\ref{item:i1} and replace the $3\times3$ convolution in the residual block with a grouped convolution. We set the group size to 16 rather than 1 (\ie depthwise convolution as in ConvNeXt) as depthwise convolution is highly inefficient on GPUs and is not much faster than using a larger group size. With grouped convolution, we can reduce the bottleneck compression ratio to two given the same model size. This increases the width of the bottleneck to $1.5\times$ as wide as Config A. 
%With this, the FID drops to 7.51, surpassing the performance of StyleGAN2. 
Finally, we notice that the compute cost of grouped convolution is negligible compared to $1\times1$ convolution, and so we seek to enhance the capacity of grouped convolution. We apply i.\ref{item:i2}), which inverts the bottleneck width and the stem width, and which doubles the width of grouped convolutions without any increase in model size. Figure~\ref{fig:network} depicts our final design, which reflects modern CNN architectures.

